A robust approach for principal component analyisis

In this paper we analyze different ways of performing principal component analysis throughout three different approaches: robust covariance and correlation matrix estimation, projection pursuit approach and non-parametric maximum entropy algorithm. The objective of these approaches is the correction of the well known sensitivity to outliers of the classical method for principal component analysis. Due to their robustness, they perform very well in contaminated data, while the classical approach fails to preserve the characteristics of the core information.

==> some.tex <==
The Reinyi's quadratic entropy of a random variable $X$ with probability density function $f_X(x)$ defined by
\begin{equation}
    \label{eq:ent}
    H(X) = -\log\int f^2_X(x) dx
\end{equation}

\begin{equation}
    \label{eq:gk}
    G(X - X_i, \sigma^2) =  \frac{1}{(2\pi)^{d/2}}\exp{\left(-\frac{||x-x_i||^2}{2\sigma^2}\right)}
\end{equation}
